On the development and analysis of coupled surface-subsurface models of catchments. Part 1. Analysis of dimensions and parameters for UK catchments

The objective of this three-part work is to formulate and rigorously analyse a number of reduced mathematical models that are nevertheless capable of describing the hydrology at the scale of a river basin (i.e. catchment). Coupled surface and subsurface flows are considered. In this first part, we identify and analyse the key physical parameters that appear in the governing formulations used within hydrodynamic rainfall-runoff models. Such parameters include those related to catchment dimensions, topography, soil and rock properties, rainfall intensities, Manning's coefficients, and river channel dimensions. Despite the abundance of research that has produced data sets describing properties of specific river basins, there have been few studies that have investigated the ensemble of typical scaling of key physical properties; these estimates are needed to perform a proper dimensional analysis of rainfall-runoff models. Therefore, in this work, we perform an extensive analysis of the parameters; our results form a benchmark and provide guidance to practitioners on the typical parameter sizes and interdependencies. Crucially, the analysis is presented in a fashion that can be reproduced and extended by other researchers, and wherever possible, uses publicly available data sets for catchments in the United Kingdom.

==> TIKZ_FIGURES/UK_map_grid.tex <==
% plotmap(x, y, filename, title, min, max)
\newcommand{\plotmap}[6] {
    \definecolor{fillColorA}{RGB}{240,249,232}
    \definecolor{fillColorB}{RGB}{186,228,188}
    \definecolor{fillColorC}{RGB}{123,204,196}
    \definecolor{fillColorD}{RGB}{67,162,202}
    \definecolor{fillColorE}{RGB}{8,104,172}
    
    \begin{scope}[xshift=#1\linewidth, yshift=#2\linewidth]
        \node[anchor=west] at (0,0)
        {\includegraphics[trim=250 0 250 90, clip, width=0.14\linewidth]{FIGURES/UK_map_grid/#3}};
        
    	\node[anchor=west,inner sep=0pt, outer sep=0pt, scale=1.0] at (0,70) {#4};
    	
    	\coordinate (A) at (18,-75);
    	\coordinate (B) at ($(A) + (12, 0)$);
    	\coordinate (C) at ($(B) + (12, 0)$);
    	\coordinate (D) at ($(C) + (12, 0)$);
    	\coordinate (E) at ($(D) + (12, 0)$);
    	\coordinate (F) at ($(E) + (12, 0)$);
    	\path[fill=fillColorA] (A) rectangle +(12,10);
    	\path[fill=fillColorB] (B) rectangle +(12,10);
    	\path[fill=fillColorC] (C) rectangle +(12,10);
    	\path[fill=fillColorD] (D) rectangle +(12,10);
    	\path[fill=fillColorE] (E) rectangle +(12,10);
    	\node[scale=0.7] at ($(A)+(0,-6)$) {#5};
    	\node[scale=0.7] at ($(F)+(0,-6)$) {#6};
    \end{scope}
}

\begin{tikzpicture}[x=1pt,y=1pt]
\plotmap{0}{0}{UK_map_grid_plot1.png}{(a) $R$ }{$1.7\cdot 10^{-8}$}{$1.1\cdot 10^{-7}$}
\plotmap{0.14}{0}{UK_map_grid_plot2.png}{(b) $Q$ }{$0$}{$1.6\cdot 10^{-7}$}
\plotmap{0.28}{0}{UK_map_grid_plot3.png}{(c) $L_z^\mathrm{all}/A$ }{$0$}{$5.8\cdot 10^{-3}$}
\plotmap{0.42}{0}{UK_map_grid_plot4.png}{(d) $L_z^\mathrm{main}/A$ }{$0$}{$1.6\cdot 10^{-3}$}
\plotmap{0.56}{0}{UK_map_grid_plot5.png}{(e) $L_x^\mathrm{stream}$ }{$140$}{$3200$}
\plotmap{0.70}{0}{UK_map_grid_plot6.png}{(f) $S_y$ }{$4.4\cdot 10^{-4}$}{$0.17$}
\plotmap{0.84}{0}{UK_map_grid_plot7.png}{(g) $S_x$ }{$8.6\cdot 10^{-3}$}{$0.45$}
\plotmap{0}{-0.3}{UK_map_grid_plot8.png}{(h) $L_z$ }{$0$}{$5700$}
\plotmap{0.14}{-0.3}{UK_map_grid_plot9.png}{(i) $K_s$ }{$7.1\cdot 10^{-8}$}{$7.7\cdot 10^{-6}$}
\plotmap{0.28}{-0.3}{UK_map_grid_plot10.png}{(j) $\alpha_\mathrm{MvG}$ }{$1.3$}{$12$}
\plotmap{0.42}{-0.3}{UK_map_grid_plot11.png}{(k) $\theta_R$ }{$0$}{$0.01$}
\plotmap{0.56}{-0.3}{UK_map_grid_plot12.png}{(l) $\theta_S$ }{$0.43$}{$0.49$}
\plotmap{0.70}{-0.3}{UK_map_grid_plot13.png}{(m) $n$ }{$1.12$}{$1.24$}
\plotmap{0.84}{-0.3}{UK_map_grid_plot14.png}{(n) $n_s$ }{$0.025$}{$0.15$}
\end{tikzpicture}
